On the Neural Tangent Kernel of Equilibrium Models

This work studies the neural tangent kernel (NTK) of the deep equilibrium (DEQ) model, a practical ``infinite-depth'' architecture which directly computes the infinite-depth limit of a weight-tied network via root-finding. Even though the NTK of a fully-connected neural network can be stochastic if its width and depth both tend to infinity simultaneously, we show that contrarily a DEQ model still enjoys a deterministic NTK despite its width and depth going to infinity at the same time under mild conditions. Moreover, this deterministic NTK can be found efficiently via root-finding.

==> linear_case_weakly_trained.tex <==
\section{Case Study: Weakly-trained Linear DEQ}

\Cref{thm:exchangelimit} shows a quite surprising result that we can safely exchange the limits, which is not at all straightforward to see. Consider the following linear DEQ case:
\[
	f_\theta^{(h)}(x) = \sqrt{\frac{\sigma_W^2}{n}}W^Tf_\theta^{(h-1)}(x)+\sqrt{\frac{\sigma_U^2}{n}}U^Tx.
\]
For simplicity, let us consider the weakly-trained network \footnote{Since we do not need to take the gradient here, we can omit the independently drawn classification layer $v\in\R^n$.}, recall the kernel that weakly-trained network induces has the following kernel:
\[
	K(x, y)=\E_{\theta}[\ip{f_\theta(x)}{f_\theta(y)}].
\]

Following the same derivation in \cref{sec:deqntk}, one can easily show that $\lim_{d\to\infty}\lim_{n\to\infty} K(x, x')=\frac{\sigma_U^2x^Ty}{1-\sigma_W^2}$. However, if we take the depth to infinity first, we have $f_\theta^*(x)=\p{I-\sqrt{\frac{\sigma_W^2}{N}W}}^{-1}\sqrt{\frac{\sigma_U^2}{N}}U^Tx$, which does not even follow a Gaussian distribution. It is not straightforward to see the limit exchange argument works. In this section, we aim to solve this weakly-trained linear DEQ case rigorously as a sanity check. We also include numerical approximation that indicates the NTK of fully-trained DEQ behaves as we expect.


\begin{theorem}
	Let $K_{d,n}(x,y)=f^{(d)}(x)^Tf^{(d)}(y)$, and $f_\theta^{(h)}(x) = \sqrt{\frac{\sigma_W^2}{n}}W^Tf_\theta^{(h-1)}(x)+\sqrt{\frac{\sigma_U^2}{n}}U^Tx$. We have
	\[
		\lim_{d\to\infty}\lim_{n\to\infty}K_{d,n}(x,y)=\lim_{n\to\infty}\lim_{d\to\infty}K_{d,n}(x,y)=\frac{\sigma_U^2x^Ty}{1-\sigma_W^2}
	\]
	almost surely.
\end{theorem}
Note that our conclusion here is even stronger than \cref{thm:exchangelimit} asserts: the latter only guarantees convergence with high probability. 

\begin{hproof}
	By definition we have 
	\begin{align*}
	\begin{split}
		&\lim_{d\to\infty}K_{d,n}(x,y)\\
		&=\frac{\sigma_U^2}{n}x^TU^T \p{I-\sqrt{\frac{\sigma_W^2}{n}W}}^{-T}\p{I-\sqrt{\frac{\sigma_W^2}{n}W}}^{-1}U^Tx\\
		&\xrightarrow{p}\sigma_U^2 x^Ty \frac{1}{n}\tr\p{\p{I-\sqrt{\frac{\sigma_W^2}{n}W}}^{-T}\p{I-\sqrt{\frac{\sigma_W^2}{n}W}}^{-1}}\\
		&\xrightarrow{} \sigma^2_Ux^Ty\int\frac{1}{\lambda}d\mu(\lambda),
	\end{split}
	\end{align*}
	where the first convergence happens with high probability \citep{arora2019exact}, and the second convergence holds for every realization of a sequence of $W$. This follows from the weak convergence of probability measure $\mu_n\xrightarrow{d}\mu$ a.s. and Portmanteau lemma, where $\mu_n$ is the empirical distribution of the eigenvalue of the matrix $\p{I-\sqrt{\frac{\sigma_W^2}{n}W}}^{T}\p{I-\sqrt{\frac{\sigma_W^2}{n}W}}$. More precisely, $\mu_n=\frac{1}{n} \sum_{i=1}^{n} \delta_{\lambda_{i}}$, $\delta_{\lambda_i}$ is the delta measure at the $i$th eigenvlue value $\lambda_i$.
	
	Now it suffices to show that $\int\frac{1}{\lambda}d\mu(\lambda)=\frac{1}{1-\sigma_W^2}$. From \citet{capitaine2016spectrum}, we learn that the Stieltjes transform of $\mu$ is a root to the following cubic equation:
	\[
		\text{For }z\in\mathbb C^+: g_\mu(z)^{-1} = \left(1- \sigma_W^{2} g_{\mu}(z)\right) z-\frac{1}{1- \sigma_W^{2} g_{\mu}(z)}.
	\]
	One could apply the inverse formula of Stieltjes transformation from here, which amounts to a very complicated integrand. Here we take a different approach and integrate the implicit equation directly. The details are deferred to the appendix. 	
\end{hproof}

The exact limiting eigenvalue distribution $\mu$ of $\sigma_W^2=0.25, 0.5, 0.75$ is shown in \cref{fig:dist_randmat}, and for $\sigma_W^2=0.25$ we include an empirical eigenvalue distribution of $\p{I-\sqrt{\frac{\sigma_W^2}{n}W}}^{T}\p{I-\sqrt{\frac{\sigma_W^2}{n}W}}$ for $n=1000$. One can see that the empirical density is very close to the limiting distribution for large enough $n$. 

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./figures/linear/dist_3cases.pdf}
	\caption{The limiting eigenvalue distribution of matrices of interest.}
	\label{fig:dist_randmat}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./figures/linear/s0.25_example.pdf}
	\caption{The empirical eigenvalue distribution of a $1000\times 1000$ instance of the random matrix.}
	\label{fig:empirical_dist_randmat}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{./figures/linear/emp_vs_theory_trace.pdf}
	\caption{The empirical and expected trace.}
	\label{fig:emp_vs_theory_trace}
\end{figure}


